Revisiting eight-manifold flux compactifications of M-theory using geometric algebra techniques

Motivated by open problems in F-theory, we reconsider warped compactifications of M theory on 8-manifolds to AdS3 spaces in the presence of a non-trivial field strength of the M-theory 3-form, studying the most general conditions under which such backgrounds preserve N=2 supersymmetry in three dimensions. In contrast with previous studies, we allow for the most general pair of Majorana generalized Killing pinors on the internal 8-manifold, without imposing any chirality conditions on those pinors. We also show how such pinors can be lifted to the 9-dimensional metric cone over the compactification 8-manifold. We describe the translation of the generalized Killing pinor equations for such backgrounds to a system of differential and algebraic constraints on certain form-valued pinor bilinears and develop techniques through which such equations can be analyzed efficiently.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
% that are currently in use and accepted by Romanian Journal of Physics.
%Last modified: 28/01/2011 (dd/mm/yyyy)

%Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}

%Various other operators
\DeclareMathOperator{\Tr}{Tr}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

%Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\cosec}{cosec}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
\providecommand{\pd}{\ensuremath{\partial}}
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}

%bras and kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
%the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}

%Commands for multiple indexes around a central token #1
%The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
%the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
%that it reduces the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}

%put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}

%A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

